Period spacings of $\gamma$ Doradus pulsators in the \textit{Kepler} field: Rossby and gravity modes in 82 stars

Rossby modes are the oscillations in a rotating fluid, whose restoring force is the Coriolis force. They provide an additional diagnostic to understand the rotation of stars, which complicates asteroseismic modelling. We report 82 $\gamma$\,Doradus stars for which clear period spacing patterns of both gravity and Rossby modes have been detected. The period spacings of both show a quasi-linear relation with the pulsation period but the slope is negative for the gravity modes and positive for the Rossby modes. Most Rossby modes have $k=-2, m=-1$. For only one star a series of $k=-1,m=-1$ modes is seen. For each pattern, the mean pulsation period, the mean period spacing, and the slope are measured. We find that the slope correlates with the mean period for Rossby mode patterns. The traditional approximation of rotation is used to measure the near-core rotation rate, assuming the star rotates rigidly. We report the near-core rotation rates, the asymptotic period spacings, and the radial orders of excited modes of these 82 main-sequence stars. The near-core rotation rates lie between $0.6\,\mathrm{d^{-1}}$ and $2.3\,\mathrm{d^{-1}}$. Six stars show surface rotation modulations, among which only KIC\,3341457 shows differential rotation while the other five stars have uniform rotations. The radial orders of excited modes show different distributions for the dipole and quadrupole gravity modes versus the Rossby modes.

==> figures/all_candidate <==
import numpy as np,os
import matplotlib.pyplot as plt
import corner
from scipy.optimize import curve_fit
#import plotly.plotly as py
def exp_func(x,a,b):
	return a*x**b

def lnlike(theta, x, y, yerr):
    m, b= theta
    model = m * x + b
    return np.sum( np.log(1/yerr)-(y-model)**2/(2*yerr**2)  )

def lnprior(theta):
    m, b = theta
    if 0 < m <2 and 3 < b < 4:
        return 0
    else:
        return -np.inf

def lnprob(theta, x, y, yerr):
    lp = lnprior(theta)
    if not np.isfinite(lp):
        return -np.inf
    return lp + lnlike(theta, x, y, yerr)

def my_period_function(n,period,delta_p,slope):
	if slope==0:slope=10**(-6.)
	#print slope
	return ((slope+1)**(n)-1)/slope*delta_p+period

filename='period_spacing_gamma_dor_table_sorted.dat'

tmp_filename='sdfsdfd'

fid=open(filename,'r')



total_information=fid.read()
fid.close()
#print total_information[1:1000]


total_information=total_information.replace('KIC & P & $\sigma_P$ & $\Delta_P$ & $\sigma_{\Delta P}$ & $\Sigma$ & $\sigma_{\Sigma}$ & N & $P_{max}$ & $P_{g}$ & $A_{g}$ \\\\','')
total_information=total_information.replace('&','').replace('\\\\','')


fid=open(tmp_filename,'w')
fid.write(total_information)
fid.close()

data=np.loadtxt(tmp_filename)
os.remove(tmp_filename)


KIC_number,P,P_err,delta_p,delta_p_err,slope,slope_err,length,P_max,P_g,A_g=data[:,0],(data[:,1]),data[:,2],(data[:,3]),data[:,4],data[:,5],data[:,6],data[:,7],data[:,8],data[:,9],data[:,10]


#get the averaged p and delta p
mean_P=np.zeros(len(P))
mean_delta_p=np.zeros(len(P))
mean_P_err=np.zeros(len(P))
mean_delta_p_err=np.zeros(len(P))
for i in range(len(KIC_number)):
	#print KIC_number[i]
	period_series=my_period_function(range(int(length[i])),P[i],delta_p[i],slope[i])
	mean_P[i]=np.mean(period_series)
	mean_delta_p[i]=np.mean(period_series[1:len(period_series)]-period_series[0:len(period_series)-1])
	print(mean_delta_p[i])
#fit p_i with i to get mean_delta_p
	tmp_para=np.polyfit(np.arange(len(period_series)), period_series, 1)
	mean_delta_p[i]=tmp_para[0]
	print(mean_delta_p[i])



	mean_P_err[i]=np.std(period_series)
	mean_delta_p_err[i]=np.std(period_series[1:len(period_series)]-period_series[0:len(period_series)-1])


from mpl_toolkits.mplot3d import Axes3D
fig=plt.figure()
ax=fig.add_subplot(111, projection='3d')
ax.scatter(np.log10(mean_P), np.log10(mean_delta_p), slope)
ax.set_xlabel('Period in d')
ax.set_ylabel('Period spacing')
ax.set_zlabel('Slope')
plt.show()



popt,pcov=curve_fit(exp_func,mean_P,mean_delta_p)
print('a*x**b, a and b:',popt)
plt.figure(figsize=(6.5,9))
ax1=plt.subplot(2,1,1)
color=slope
#ax.errorbar(P,delta_p,xerr=P_err,yerr=delta_p_err,fmt=',')
sc=ax1.scatter(mean_P,mean_delta_p*86400,c=color,lw=0,s=50)
plt.colorbar(sc,label='Slope')
ax1.set_ylim([0,10000])
ax1.set_xlabel('<P> in d')
ax1.set_ylabel('<$\Delta$P> in s')
#lower limit of resolution
ax1.plot(np.linspace(0.2,2,100),0.0007*np.linspace(0.2,2,100)**2*86400*4,'r-.')
#radial order n
for n_times in np.array([400,200,100,50,25,12]):
	ax1.plot(np.linspace(0.2,2,100),1.0/n_times*np.linspace(0.2,2,100)*86400,'g--')
	if n_times !=12:
		ax1.text(2,1.0/n_times*2*86400,str(n_times))
	else:
		ax1.text(1.12,8854,'$\langle P \\rangle / \langle \Delta P \\rangle$='+str(n_times))



#logarithm axis
ax2=plt.subplot(2,1,2)
color=slope
#ax.errorbar(np.log10(P),np.log10(delta_p),xerr=P_err/(P*np.log(10)),yerr=delta_p_err/(delta_p*np.log(10)),fmt=',')
sc=ax2.scatter(np.log10(mean_P),np.log10(mean_delta_p*86400),c=color,lw=0,s=50)
plt.colorbar(sc,label='Slope')
ax2.set_ylim([1.5,4.0])
ax2.set_xlabel('log<P>')
ax2.set_ylabel('log<$\Delta$P>')
ax2.plot(np.log10(np.linspace(0.2,2,100)),np.log10(0.0007*np.linspace(0.2,2,100)**2*86400*5),'r-.')
for n_times in np.array([400,200,100,50,25,12]):
	ax2.plot(np.log10(np.linspace(0.2,2,100)),np.log10(1.0/n_times*np.linspace(0.2,2,100)*86400),'g--')
	if n_times !=12:
		ax2.text(0.3,np.log10(1.0/n_times*2.0*86400),str(n_times))
	if n_times==12:
		ax2.text(-0.2,3.76,'$\langle P \\rangle / \langle \Delta P \\rangle$='+str(n_times))

plt.subplots_adjust(left=0.14, bottom=0.07, right=0.95, top=0.97, wspace=0.20, hspace=0.18)
plt.savefig('/export/pushkin1/gali8292/project1/paper/my_paper/period_periodspacing_slope.pdf')
#linear fit to log_P and log_delta_p
linear_para=np.polyfit(np.log10(mean_P),np.log10(mean_delta_p*86400),1)
#ax2.plot(np.sort(np.log10(mean_P)),np.polyval(linear_para,np.sort(np.log10(mean_P))))
print('linear fit result',linear_para)
print('linear_fit_residual',np.std(np.log10(mean_delta_p)-np.polyval(linear_para,np.log10(mean_P))))
print('no_fit_residual',np.std(np.log10(mean_delta_p)))


plt.figure()
color=A_g**0.25
sc=plt.scatter(P_max,P_g,c=color,lw=0)
plt.plot(np.sort(P_max),np.sort(P_max),'r')
plt.colorbar(sc)
plt.xlabel('P_max')
plt.ylabel('P_g')
#print dir(ax)
#print ax.axes,len(ax.axes)
#ax.axes[4].set_xlim([0,4000])
#ax.axes[7].set_xlim([0,4000])
#ax.xlim([0,3])

#plot hist by myself
plt.figure()
hist1=plt.subplot(2,2,1)
hist1.hist(mean_P,bins=20,color='grey')
hist1.set_xlabel('P in d')
hist1.set_ylabel('Number')
hist2=plt.subplot(2,2,2)
hist2.hist(mean_delta_p*86,bins=20,color='grey')
hist2.set_xlabel('$\Delta$P in 1000 s')
hist3=plt.subplot(2,2,3)
hist3.hist(slope,bins=20,color='grey')
hist3.set_xlabel('Slope')
hist3.set_ylabel('Number')
hist3.set_xlim([-0.2,0.3])
hist4=plt.subplot(2,2,4)
hist4.hist(length,bins=20,color='grey')
hist4.set_xlabel('Pattern length')

plt.subplots_adjust(left=0.08, bottom=0.09, right=0.97, top=0.97, wspace=0.10, hspace=0.26)
plt.savefig('/export/pushkin1/gali8292/project1/paper/my_paper/4_parameters_distributions.pdf')

print('The percentage that the slope <0', float(len(np.where(slope<0)[0]))/len(slope))

#plot hist for amplitude
plt.figure()
hist1=plt.subplot(3,1,1)
hist1.hist(A_g,bins=40,range=(0,0.004))
hist2=plt.subplot(3,1,2)
hist2.hist(mean_P/mean_delta_p,bins=40,range=(15,200))
hist3=plt.subplot(3,1,3)
hist3.plot(mean_P/mean_delta_p,A_g,'.')
#plt.show()
#emcee

ndim, nwalkers, chain_step = 2, 10, 1000
pos = [[1.08,3.14] + 0.01*np.random.randn(ndim) for i in range(nwalkers)]

import emcee
sampler = emcee.EnsembleSampler(nwalkers, ndim, lnprob, args=(np.log10(mean_P),np.log10(mean_delta_p*86400), mean_delta_p_err/mean_delta_p/np.log(10) ) )
plt.show()
sampler.run_mcmc(pos, chain_step)
samples = sampler.chain[:, 50:, :].reshape((-1, ndim))

length=len(samples[:,0])

MCMC_slope=np.sort(samples[:,0])
MCMC_intercept=np.sort(samples[:,1])
print('MCMC results,the slope',MCMC_slope[int(0.5*length)],MCMC_slope[int(0.84*length)]-MCMC_slope[int(0.5*length)],MCMC_slope[int(0.5*length)]-MCMC_slope[int(0.16*length)])
print('MCMC results,the intercept',MCMC_intercept[int(0.5*length)],MCMC_intercept[int(0.84*length)]-MCMC_intercept[int(0.5*length)],MCMC_intercept[int(0.5*length)]-MCMC_intercept[int(0.16*length)])

#ax2.plot(np.sort(np.log10(mean_P)),MCMC_slope[int(0.5*length)]*np.sort(np.log10(mean_P))+MCMC_intercept[int(0.5*length)],'r')

import corner
fig = corner.corner(samples, labels=["The slope", "The intercept"],quantiles=[0.16,0.5,0.84])



#plt.show()
#find something about Metallicity, radius, log_g, T_eff

the_document=open('kepler_search(5).txt','r').readlines()

#print the_document[2].split(",")

for i in range(len(the_document[0].split(","))):
	print(i, the_document[0].split(",")[i])

#plt.show()

spec_data=np.zeros([len(the_document)-2,len(the_document[2].split(","))])

for line_counter in range(len(the_document)-2):
	data_element=the_document[line_counter+2].split(",")
	for i in range(len(data_element)):
		if data_element[i]=='':
			data_element[i]='9999'
		spec_data[line_counter,i]=float(data_element[i])
#os.system('rm tmp_file')

#print spec_data


plt.figure()
plt.hist(spec_data[:,1])

index=[]
index_for_spec_data=[]
for i in range(len(spec_data)):
	#print 'KIC number in spec data', spec_data[i,0]
	if np.min(  np.abs(spec_data[i,0]-KIC_number))  ==0 and min(np.abs(spec_data[i,:]-9999))!=0:
		#print np.where(spec_data[i,0]==KIC_number)[0]#np.argmin(  np.abs(spec_data[i,0]-KIC_number))
		#print np.where(spec_data[i,0]==KIC_number)[0]
		for tmp_element in np.where(spec_data[i,0]==KIC_number)[0]:
			index.append( tmp_element )
			index_for_spec_data.append(i)
	#tmp_index=np.where(spec_data[i,0]==KIC_number)[0]

print(len(index))
index=np.array(index)
index_for_spec_data=np.array(index_for_spec_data)
plt.figure()
log_mean_P,log_mean_delta_p=np.log10(mean_P[index]),np.log10(mean_delta_p[index]*86400)
ax1=plt.subplot(1,1,1)
#color=(mean_delta_p[index])
#color=mean_P[index]
color=slope[index]
#ax1.plot(np.log10(spec_data[index_for_spec_data,12]),slope[index],'.')
#ax1.plot(spec_data[index_for_spec_data,6],mean_delta_p[index],'.')
#ax1.plot(spec_data[index_for_spec_data,3]-spec_data[index_for_spec_data,4],spec_data[index_for_spec_data,6],'.')
#ax1.plot(spec_data[index_for_spec_data,7],spec_data[index_for_spec_data,12],'.')
#ax1.set_xlim([8500,5500])

ax1.scatter(spec_data[index_for_spec_data,9],spec_data[index_for_spec_data,12],c=color,lw=0,s=50)
#ax1.set_xlim([8500,5500])

#plt.colorbar(sc)

















plt.show()


